Collaborative Evolution: Multi-Round Learning Between Large and Small Language Models for Emergent Fake News Detection

The proliferation of fake news on social media platforms has exerted a substantial influence on society, leading to discernible impacts and deleterious consequences. Conventional deep learning methodologies employing small language models (SLMs) suffer from the necessity for extensive supervised training and the challenge of adapting to rapidly evolving circumstances. Large language models (LLMs), despite their robust zero-shot capabilities, have fallen short in effectively identifying fake news due to a lack of pertinent demonstrations and the dynamic nature of knowledge. In this paper, a novel framework Multi-Round Collaboration Detection (MRCD) is proposed to address these aforementioned limitations. The MRCD framework is capable of enjoying the merits from both LLMs and SLMs by integrating their generalization abilities and specialized functionalities, respectively. Our approach features a two-stage retrieval module that selects relevant and up-to-date demonstrations and knowledge, enhancing in-context learning for better detection of emerging news events. We further design a multi-round learning framework to ensure more reliable detection results. Our framework MRCD achieves SOTA results on two real-world datasets Pheme and Twitter16, with accuracy improvements of 7.4\% and 12.8\% compared to using only SLMs, which effectively addresses the limitations of current models and improves the detection of emergent fake news.

==> Table/ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Ablation Study on Three Datasets}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{l|rrrr|rrrr|rrrr}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{Variant Models}} & \multicolumn{4}{c|}{Pheme}    & \multicolumn{4}{c|}{Twitter}  & \multicolumn{4}{c}{Weibo} \\
\cmidrule{2-13}          & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c}{F1} \\
    \midrule
    \zzy{xxx(Lamma3-Based)} &0.788       &0.700       & 0.900      & 0.786      & 0.772      & 0.765      &0.775       & 0.770      & 0.712      & 0.753      & 0.802      & 0.777 \\
    \midrule
    w/o Demonstration & 0.762      & 0.691      & 0.920      &0.774      & 0.680      & 0.808      & 0.675      &0.683      &       &       &       &  \\
    \textit{w/o Search Engine} &0.774       &0.712       & 0.850      &0.771        &0.763       & 0.754      & 0.761      & 0.756&         &       &       &  \\
    \textit{w/o News Corpus}&0.772       & 0. 691     &0.883       &0.778 &0.758       &  0.765     & 0.782      &0.761  &                  &       &       &  \\
    \midrule
    w/o Knowledge & 0.769      &  0.695     & 0.831      &  0.752     &0.761       &0.762       &0.734       &0.748       &       &       &       &  \\
    % w/o SLM &       &       &       &       &       &       &       &       &       &       &       &  \\
    w/o Multi-Round &\zzy{0.717}       &0.702      &  0.789     & 0.741      & 0.678      & 0.662      &0.704       &0.691       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:ablation}%
\end{table}%


==> Table/dataset.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Details of three datasets.}
    \begin{tabular}{l|r|r|r}
    \toprule
    Dataset & \multicolumn{1}{l|}{Twitter16} & \multicolumn{1}{l|}{Pheme} & \multicolumn{1}{l}{Weibo} \\
    \midrule
    Train &       &       &  \\
    \midrule
    Val   &       &       &  \\
    \midrule
    Test(Fake) &       &       &  \\
    \midrule
    Test(Real) &       &       &  \\
    \end{tabular}%
  \label{tab:dataset}%
\end{table}%


==> Table/main_ex.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \caption{Performance of XXX. Best Results are in \textbf{bold} and second best results are \underline{underlined} }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|rrrr|rrrr|rrrr}
    \toprule 
    \multirow{2}[4]{*}{Category} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Method}} & \multicolumn{4}{c|}{Pheme} & \multicolumn{4}{c|}{Twitter} & \multicolumn{4}{c}{\zzy{Weibo}} \\
\cmidrule{3-14}    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c}{F1} \\
    \midrule
    \multirow{3}[2]{*}{SLM} & \zzy{RoBERTa}  & 0.714      & 0.777      & 0.695      & 0.734      &0.644       &0.649       &0.641       &0.645       &       &       &       &  \\
          & EANN  & 0.744      & 0.738      & 0.745      & 0.741      & 0.641      & 0.621      & 0.741      & 0.676      &  0.889     & 0.674      & 0.820      & 0.740 \\
          & M$^{3}$FEND &  0.746     & 0.747      & 0.746      & 0.746      & 0.642      & 0.608      & 0.816      & 0.697      & 0.896      & 0.715      & 0.801      & 0.761 \\
    \midrule
    \multirow{3}[2]{*}{\makecell[l]{LLM \\ (zero-shot)}} & Lamma2-7B &0.505       & 0.498      & 0.697      & 0.581      &0.496       &0.501       &0.494        &0.498 &       &       &       &        \\
    & Lamma3-8B & 0.535   & 0.518     & 0.770      & 0.620      &  0.562     & 0.574      &  0.531     &  0.552     & 0.579      & 0.442      &0.651       &0.527  \\
          & gpt3.5 &0.503       & 0.500      &  0.714     &0.586       & 0.633      &0.655       & 0.584      & 0.618      &       &       &       &  \\
    \midrule
    \multirow{3}[2]{*}{\makecell[l]{LLM \\ (few-shot)}}
          & Lamma2-7B & 0.528      &0.511       &0.894       &0.650       &0.590       &0.598       &0.584       & 0.591      &       &       &       &  \\
          & Lamma3-8B & 0.549      &0.524       & 0.961      & 0.679      & 0.622      &0.607       & 0.717      &   0.658    &  0.597     & 0.466      &0.827       & 0.600 \\
          & \zzy{gpt3.5} &0.520       & 0.507      & 0.850      &0.635       &0.621       & 0.609      & 0.705      &0.653       &       &       &       &  \\
    \midrule
    LLM+SLM & ARG  &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multirow{4}[2]{*}{Ours} & Lamma2-Based &0.772       &0.765       &0.775       &0.770       &0.732       &0.717       & 0.619      & 0.664 &      &       &       &        \\
          & Lamma3-Based  &0.788       & 0.700      & 0.900      &0.786  &0.772       &0.765       &0.775       &0.770       &       &       &      & \\
          & Gpt3.5-Based  &0.781       & 0.735      &0.821       &0.778      &0.768       &0.752       & 0.734      & 0.761      &       &       &       &  \\
    & \textit{Impr. RoBERTa} & +\textit{6.7\%}      & /      &  +\textit{20.5\%}     & +\textit{5.2\%}      & +\textit{12.4\%}     &+\textit{11.6\%}       & +\textit{13.4\%}     & +\textit{12.5\%}      &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{main_ex}%
\end{table*}%


==> Table/wrap_dataset.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{wraptable}[l]{0.5\textwidth}
  \caption{Details of three datasets.}
    \begin{tabular}{l|r|r|r}
    \toprule
    Dataset & \multicolumn{1}{l|}{Twitter16} & \multicolumn{1}{l|}{Pheme} & \multicolumn{1}{l}{Weibo} \\
    \midrule
    Train &       &       &  \\
    \midrule
    Val   &       &       &  \\
    \midrule
    Test(Fake) &       &       &  \\
    \midrule
    Test(Real) &       &       &  \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{wraptable}%


==> code/alg1.tex <==
\begin{algorithm}[!t]
% \begin{algorithm}[H]
% \fontsize{7pt}{1pt}
% \setstretch{0.15}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
  \Input{Emergent Events $\{X_e^t\} = \{x_{e,i}^t\}_{i=K+1}^N$, LLM $\mathcal{L}$, SLM $\mathcal{S}$ initialized with Past Events $\{X_e^s,Y_e^s\} = \{x_{e,i}^s,y_{e,i}^s\}_{i=1}^K$, round $=$ 1}
  \Output{Labeled Emergent Events $\{X_e^t\} = \{x_{e,i}^t,y_{e,i}^t\}_{i=K+1}^N$}
  % \BlankLine
  % \emph{Initialize parameters for $\mathcal{S}$ with past events data  $\{X_e^s,Y_e^s\}$}\;
  \tcc{Multi-round Learning}\
  % round = 1\;
  \If{round == 1}{
    % Retrieve relevant news $(N_w,N_c)$ from  $\mathcal{W}$ and  $\mathcal{C}$\;
    Obtain Demonstrations $\mathcal{D}$ by BM25 and assign pseudo labels from $(\mathcal{W},\mathcal{C})$;\\
    Knowledge-Retrieval Module to obtain $\mathcal{K}$;\\
    Inference by $\mathcal{L}$ and $\mathcal{S}$ to obtain $(\widehat{y_1},\widehat{y_2})$: \\
    $ \widehat{y_1}=argmax_{\widehat{y_1} \in \mathcal{Y}}P(\widehat{y_1}| \mathcal{D},\mathcal{K},x)  \\ \widehat{y_2}=argmax_{\widehat{y_2} \in \mathcal{Y}}P(\widehat{y_2}|x)$
    ; \\
    Data selection model to obtain  $D_{clean}$ and $D_{noisy}$; \\
    round = round + 1;
  }
  \For {round $\leq$ $\mathcal{N}$}{
  % \tcc{Reinforced propagation path generation}
    % Obtain $\mathcal{D}$ by retrieving from $D_{clean}$\;
    % Fine-tune $\mathcal{S}$ with $D_{clean}$\;
    Retrieve  $\mathcal{D}$ for $\mathcal{L}$ and fine-tune $\mathcal{S}$ by $D_{clean}$; \\
     $D_{noisy}$ inference by $\mathcal{L}$ and $\mathcal{S}$ to obtain $(\widehat{y_1},\widehat{y_2})$; \\
     Data selection module to update $D_{clean}$ and $D_{noisy}$; \\
     round = round + 1;
  }
  \If{$D_{noisy} \neq \emptyset$}{
    $D_{noisy}$ inference by $\mathcal{S}$ to obtain $\widehat{y_2}$; \\
    Update $D_{clean}$ as final labels;
  }
\caption{Pseudo-code for \textbf{MRCD}}
\label{alg1}
\end{algorithm}
\vspace{-6mm}
\end{figure}

==> code/alg1_halfcolumn.tex <==
\begin{figure}[!t]
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
% \fontsize{7pt}{1pt}
% \setstretch{0.15}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
  \Input{Past Events $\{X_e^s,Y_e^s\} = \{x_{e,i}^s,y_{e,i}^s\}_{i=1}^K$,  Emergent Events $\{X_e^t\} = \{x_{e,i}^t\}_{i=K+1}^N$, LLM $\mathcal{L}$, SLM $\mathcal{S}$}
  \Output{Labeled Emergent Events $\{X_e^t\} = \{x_{e,i}^t,y_{e,i}^t\}_{i=K+1}^N$}
  % \BlankLine
  \emph{Initialize parameters for $\mathcal{S}$ with past events data  $\{X_e^s,Y_e^s\}$}\;
  \tcc{Multi-round Learning}\
  round = 1\;
  \If{round == 1}{
    Retrieve relevant news $(N_w,N_c)$ from  $\mathcal{W}$ and  $\mathcal{C}$\;
    Generate Demonstrations $\mathcal{D}$ by BM25 and pseudo labels from $(N_w,N_c)$\;
    Knowledge-Retrieval Module to obtain $\mathcal{K}$\;
    Inference by $\mathcal{L}$ and $\mathcal{S}$ to obtain $(\widehat{y_1},\widehat{y_2})$: \\
    $ \widehat{y_1}=argmax_{\widehat{y_1} \in \mathcal{Y}}P(\widehat{y_1}|D,K,x) , \widehat{y_2}=argmax_{\widehat{y_2} \in \mathcal{Y}}P(\widehat{y_2}|x)$
    \;
    Data selection model to obtain clean data $D_{clean}$ and noisy data $D_{noisy}$\;
    round = round + 1\;
  }
  \For {round $\leq$ $\mathcal{N}$}{
  % \tcc{Reinforced propagation path generation}
    Retrieve from $D_{clean}$ to obtain $\mathcal{D}$\;
    Fine-tune $\mathcal{S}$ with $D_{clean}$\;
     $D_{noisy}$ inference by $\mathcal{L}$ and $\mathcal{S}$ to obtain $(\widehat{y_1},\widehat{y_2})$\;
     Data selection module to update $D_{clean}$ and $D_{noisy}$\;
     round = round + 1\;
  }
  \If{$D_{noisy} \neq \phi$}{
    $D_{noisy}$ inference by LLM to obtain $\widehat{y_1}$\;
    Update $D_{clean}$ as final labels\;
  }
\caption{Pseudo-code for \zzy{XXX}}
\label{alg1}
\end{algorithm}
\end{minipage}
% \vspace{-9mm}
\end{figure}

